Measuring Internet Routing from the Most Valuable Points

While the increasing number of Vantage Points (VPs) in RIPE RIS and RouteViews improves our understanding of the Internet, the quadratically increasing volume of collected data poses a challenge to the scientific and operational use of the data. The design and implementation of BGP and BGP data collection systems lead to data archives with enormous redundancy, as there is substantial overlap in announced routes across many different VPs. Researchers thus often resort to arbitrary sampling of the data, which we demonstrate comes at a cost to the accuracy and coverage of previous works. The continued growth of the Internet, and of these collection systems, exacerbates this cost. The community needs a better approach to managing and using these data archives. We propose MVP, a system that scores VPs according to their level of redundancy with other VPs, allowing more informed sampling of these data archives. Our challenge is that the degree of redundancy between two updates depends on how we define redundancy, which in turn depends on the analysis objective. Our key contribution is a general framework and associated algorithms to assess redundancy between VP observations. We quantify the benefit of our approach for four canonical BGP routing analyses: AS relationship inference, AS rank computation, hijack detection, and routing detour detection. MVP improves the coverage or accuracy (or both) of all these analyses while processing the same volume of data.

==> body.tex <==
\section{Introduction}


==> case_mvp.tex <==
\section{The case for \name}
\label{sec:mvp}

We demonstrate the value of strategic selection of VPs from
\ris and \rv (\S\ref{sec:problems}) and show the opportunity 
offered by redundancy in the data (\S\ref{sec:opportunity}) 
that \name leverages (\S\ref{sec:challenges}).


\subsection{Problem}
\label{sec:problems}


Deploying more VPs expands visibility of the routing system
(\S\ref{sec:case1}), but also dramatically increases collected data
volumes. We show the overwhelming quantity of data raises barriers to its use (\S\ref{sec:problem2}) leading to arbitrary sampling, with surveyed authors fearing a negative impact on the quality of their results (\S\ref{sec:problem3}).


\vspace{-0.15cm}
\subsubsection{Deploying more VPs improves data completeness.}\hfill%
\label{sec:case1}




A tiny fraction (1.3\%) of the 74k ASes participating in the global
routing system~\cite{cidr_report} host a VP.
This fraction remains low (8.4\%) even when focusing on the 11441 transit ASes (\ie those that have at least one customer).  
Although we cannot
know how much additional topology we might observe from VPs that do not
peer with the public collection systems,
we can estimate this gap using simulations of topologies
whose statistical parameters match those of the known global Internet.


\myitem{Methodology.}
We created a mini-Internet with 600 ASes, each running a single BGP
router.  We generated the AS topology using the Hyperbolic Graph
Generator~\cite{ALDECOA2015492}. We set the average node degree to 6.1,
which results in a comparable degree of connectivity (\textit{a.k.a.}
Beta index) to the one observed in CAIDA's AS relationship dataset
from December 2022~\cite{CAIDA_relationships}, and use as the 
degree distribution
a power law with exponent 2.1 (as in~\cite{ALDECOA2015492}).  We defined
the AS relationships as follows. The three ASes with the highest degree
are Tier1 ASes and are fully meshed. ASes directly connected to a Tier1
are Tier2s.  ASes directly connected to a Tier2 but not to a Tier1 are
Tier3s, etc. Two connected ASes have a peer-to-peer (p2p) relationship
if they are on the same level, a customer-to-provider (c2p) relationship
if not.  The routing policies follow the Gao-Rexford model~\cite{GaoRexford}.




\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/mini_internet-crop.pdf}
    \caption{Simulations with a 600-ASes mini-Internet from which we make two key observations:
    \first deploying more VPs helps observing more AS links (especially p2p links), and \second
    arbitrarily selecting VPs performs poorly compared to selecting them with \textit{greedy specific} (a best-base approximation). }
    \label{fig:mini-internet_exp}
\end{figure}%

\fref{fig:mini-internet_exp} shows the proportion of observed AS links
as a function of the number of ASes hosting a VP. We consider 
three VP deployment strategies: \first \textit{random}, which randomly deploys VPs across all the ASes;
\second \textit{distance-based}, which aims to maximize the AS-level distance between the deployed VPs; and \third
\textit{greedy specific}, which approximates the best case using a greedy approach.
We ran every selection strategy twenty times (with different random seeds) and show the results in the boxes.
The line in a box depicts the
median value; the whiskers show the 5 and the 95th percentile.
We computed the proportion of observed links and show separately the 
p2p and 
c2p links in \fref{fig:mini-internet_exp}. 

\myitem{Conclusions.}
Although we take the results with a grain of salt
because the topology differs (but exhibits similar patterns) from the visible portion of the actual (unknown) AS topology, we tentatively draw the following five conclusions.

\noindent
\Firstp For a given VP deployment strategy, more VPs often leads to more
links observed and all links are observed only when all ASes host a VP.
This result is intuitive as combining local views helps to gather more routing information (see \S\ref{sec:background}).

\noindent
\Secondp P2p links are harder to observe than c2p links.
After investigation, we observe that they are more visible from VPs at the edge,
which aligns with the scenarios depicted in \fref{fig:partial_view}.
Again, this result is intuitive as, unlike c2p links, p2p links are 
not expected to be advertised upwards in the Internet hierarchy when routing policies follow the Gao-Rexford model.

\noindent
\Fourthp The \textit{distance-based} deployment strategy performs poorly (even worse than random deployment).

\noindent
\Fifthp When 1.3\% of ASes host a VP (\ie the same proportion 
as current \ris and \rv VPs), %
only 35\% of the links are observed.

\myitem{Confirmation with real (but private) data.} We contacted a private BGP
data provider that collects BGP routes from $\approx$1000 routers and 
compared the set of AS links observed from these private feeds against the set of AS links 
observed by \ris and \rv VPs (as of September 2023). We find that 
the private data provider sees X AS links that \textit{none} of the \ris and \rv VPs observe, 
and vice versa, \ris and \rv VPs observe X links that the private data provider do not observe.
In either cases, the lack of VPs leads to missing routing information.

\myitem{Key takeaway.}
Our conclusions suggest that
deploying more VPs improves visible coverage of the routing topology.
Consequently, new deployments of VPs by \ris and \rv can be beneficial,
and we can expect---and hope for---their number to keep increasing (see \fref{fig:ris_nb_vp2}).





\vspace{-0.15cm}
\subsubsection{The increasing volume of data complicates data usability.}\hfill%
\label{sec:problem2}


Deploying more VPs generates more data as each of them collects BGP updates.
Moreover, new IP prefixes advertised in BGP (see~\cite{cidr_report})
increase the volume of data collected by every VP.
In fact, every new IP prefix advertised in BGP triggers the propagation of
new BGP routes that many VPs (\eg the full feeders) observe
and send to the collection platforms.
The compound effect---more VPs (\fref{fig:ris_nb_vp2})
and more updates per VP (\fref{fig:update_vp2})---yields 
a \textit{quadratic} increase in updates reaching the 
collection platforms (\fref{fig:ris_nb_updates}),
which concerns users and data providers~\cite{aben_concern}.
Although several tools aims to speed up the data processing~\cite{bgpstream,bgpkit,9464008},
our literature review revealed that many studies used only a
sample of data collected by \ris and \rv, either using only a subset of the VPs
or a short duration of time, or both.
While authors do not typically explain why they do not use all the data,
the sampling suggests two (inter-related) explanations: authors believe the
sample is representative and sufficiently complete; and/or the data volume is
not worth trying to manage.
We confirm that this is the common behaviors with a survey
that we conducted involving authors of ten research papers.  















\myitem{Methodology.} We classified ten BGP-based studies from top
conferences\footnote{SIGCOMM, NSDI, S\&P, USENIX Security, NDSS and IMC. }
into two categories based on how they used BGP data.\footnote{A
	paper may be in both categories.}
Seven papers used \textbf{all} routes collected from 
a \textbf{subset} of the VPs (category $C_1$);  
five papers used a \textbf{short time frame} ($C_2$).
\cristel{How many respondents in $C_1$ and $C_2$?}
For each paper, we asked the authors questions regarding
their use of BGP data: whether data volume limited their work, 
how and why they sampled BGP data sources, their understanding of
the impact on the quality of their results, and if they would do 
things differently if they had more resources or time.  
We summarize results here; details of the survey are in
an appendix (\S\ref{sec:survey}).

\myitem{The volume of BGP data to process is often a limiting factor.}
Seven (of 9) respondents found the BGP data expensive to process.
For three respondents in $C_1$, processing time motivated them
to use only a subset of the VPs; three respondents in $C_2$ 
considered the processing time when choosing a measurement interval.
Even a respondent that used a Spark cluster found it 
inhibitively time-consuming to process the BGP data. 

\myitem{Respondents in $C_1$ selected VPs somewhat arbitrarily.}
One respondent picked geographically-distant BGP collectors.
Our experiments
(\fref{fig:mini-internet_exp}) and our evaluation (\S\ref{sec:eval})
show that this intuitive strategy often fails to optimize for a \cristel{a -> any?}given
metric, such as coverage.  Other respondents said they chose VPs randomly,
or those with the highest number of prefixes.  Another responded to have
unintentionally discarded some VPs, leaving an arbitrarily selected set
in the study.  Two respondents did not remember how they selected VPs.


\vspace{-0.15cm}
\subsubsection{Current practices negatively impact results.}
\label{sec:problem3}


We show using our controlled simulations and our survey that current
practices to reduce the volume of data to process negatively impact the
quality of the results.

\myitem{Selecting VPs arbitrarily performs poorly.}
Our mini-Internet simulation (\S\ref{sec:case1})
shows that arbitrary VPs selection strategies
perform significantly worse than \textit{greedy specific} (a best-case 
approximation) when the goal is to map the AS topology.
For instance, randomly selecting 20 VPs reveals 12\% of the p2p links compared 
to 56\% when selecting them using \textit{greedy specific}---a 4.7$\times$ improvement factor that we highlight in \fref{fig:mini-internet_exp}.
Our evaluation reveals that this performance gap between using an arbitrary VPs selection
strategy and a best-case approach also exists for various other metrics,
\eg hijacks or transient paths detection (\S\ref{sec:eval}).


\myitem{Six respondents in $C_1$ acknowledged that using more VPs would 
improve the quality of their analysis.}
The last respondent was not sure, given the potential redundancy in
the data sources (which he did not analyze). 
Two of the six believed it would not {\em significantly} change 
the conclusion of their measurement studies
(\eg one said that it could help to pinpoint corner cases).
However, six of the 7 authors in $C_1$ affirmed that they would have
used more VPs if they had more resources and time.
\cristel{this does not mean they would reach better results with more data.}


\myitem{All respondents in $C_2$ said that extending the duration of
their study would improve the quality of their results.}
One respondent thought the gain would not be significant;
another said it could help detect rare routing events. 
All respondents in $C_2$ would have extended the duration 
of their observation window given more time and resources. 
We experimentally confirm in \S\ref{sec:eval_detours} that extending 
the timeframe of an analysis improves the quality of its results 
with a case study on routing detours characterization~\cite{forwarding-detour}.














\subsection{Opportunity to Optimize Sampling}
\label{sec:opportunity}

We now propose a systematic framework to characterize
{\em redundancy} across BGP routes collected by the VPs.  
We use the term {\em redundant} to refer to updates with 
similar (or identical, depending on the \textit{redundancy} definition)
attribute values (\S\ref{sec:opportunity1}).
Thus, two redundant VPs, \ie that observe
redundant routes, likely provide similar views over
routing events such as outages, attacks, etc.  \name exploits this
opportunity to identify a set of nonredundant VPs which collects a compound of BGP updates
with a low level of redundancy (\S\ref{sec:opportunity2}).
\kc{i think the precise defn should be something like
"yields the same inference of scope and duration 
of an inferred harm"..}



\vspace{-0.15cm}
\subsubsection{The VPs of \ris and \rv collect redundant routes}
\label{sec:opportunity1}

\setlist{leftmargin=3mm}


We characterize redundancy between pairs of VPs using three different, gradually stricter, 
definitions of redundancy.
We denote $v_i$ the VP $i$ that observes
a set of BGP updates $U_i$. Consider a BGP update $u_{t,p} \in U_i$
with $t$ the time at which the route was observed and $p$ its prefix.
\begin{defn}[prefix based]
    The update $u_{t_1,p_1} \in U_1$ is redundant with the update $u_{t_2,p_2} \in U_2$ if:
    \begin{itemize}
        \setlength\itemsep{-0.1cm}
        \item $\lvert t_1 - t_2 \lvert < 5$ minutes, and $p_1 = p_2$.
   \end{itemize}
    \label{def:red1}
  \end{defn}
\noindent
We choose 5 minutes because it is an approximation of the BGP convergence time~\cite{transientConv}.
We now denote $A_i(t,p)$ the set of AS links in the AS path of the most recent BGP route observed by 
VP $i$ for prefix $p$ at time $t$.
This definition of redundancy might be appropriate when one is merely trying to map as many routed prefixes as possible during a given time window to some AS originating them into the Internet, i.e., path diversity is not of interest. 
\begin{defn}[prefix and as-path based]
    The update $u_{t_1,p_1} \in U_1$ is redundant with the update $u_{t_2,p_2} \in U_2$ if:
    \begin{itemize}
        \setlength\itemsep{-0.1cm}
        \item $\lvert t_1 - t_2 \lvert < 5$ minutes, and $p_1 = p_2$, and
        \item $A_1(t_1, p_1) \setminus A_1(t_1-\epsilon, p_1) \subset A_2(t_2, p_2) \setminus A_2(t_2-\epsilon, p_2)$.
   \end{itemize}
   \label{def:red2}
\end{defn}
\noindent
More casually, the second condition checks whether the changes (operator $\setminus$)
in the AS paths observed by VP $1$ for a given prefix coincide (operator $\subset$) 
with the changes observed by VP $2$ for the same prefix. 

The last definition 
follows the same approach, but adding BGP communities.
We denote $C_i(t,p)$ the set of community values of the most recent BGP route observed by 
VP $i$ for prefix $p$ and at time $t$.
\noindent
\begin{defn}[prefix, as-path, and community-based]
    The update $u_{t_1,p_1} \in U_1$ is redundant with update $u_{t_2,p_2} \in U_2$ if:
    \begin{itemize}
        \setlength\itemsep{-0.1cm}
        \item $\lvert t_1 - t_2 \lvert < 5$ minutes, and $p_1 = p_2$, and
        \item $A_1(t_1, p_1) \setminus A_1(t_1-\epsilon, p_1) \subset A_2(t_2, p_2) \setminus A_2(t_2-\epsilon, p_2)$, and
        \item $C_1(t_1, p_1) \setminus C_1(t_1-\epsilon, p_1) \subset C_2(t_2, p_2) \setminus C_2(t_2-\epsilon, p_2)$.
   \end{itemize}
   \label{def:red3}
\end{defn}
We note that these definitions are asymmetric. 

\myitem{Redundant pairs of VPs exist.}
\fref{fig:redundancy} shows the level of redundancy for the three definitions and
between 100 VPs selected using three different strategies
and computed over the updates observed during two hours on August 1, 2022.
One cell in the matrix indicates the redundancy of the VP on the ordinate with the VP on the abscissa.
We define the redundancy between VP $v_1$ and VP $v_2$ as the proportion of updates observed 
by $v_1$ that are redundant with at least one update observed by $v_2$.
For better visibility, we show the most redundant VPs at the top of the figures.

\fref{fig:redundancy} illustrates that redundant pairs of VPs exist regardless 
of the redundancy definition used. Logically, the stricter the definition, the fewer redundant pairs of VPs.






\begin{figure}[t!] %


    \begin{subfigure}{0.05\textwidth}
        \includegraphics[width=\textwidth]{figures/white.png}
        
    \end{subfigure}
    \begin{subfigure}{0.38\textwidth}
        \hspace{-10cm}

        \includegraphics[width=\textwidth]{figures/redundancy_colorbar-crop.pdf}
    \end{subfigure}
    \hspace{0.5cm}
        
    \medskip

    \begin{subfigure}{0.015\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_title_vert1-crop.pdf}
        
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
    \includegraphics[width=\textwidth]{figures/redundancy_random_1-crop.pdf}
    
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}

        \includegraphics[width=\textwidth]{figures/redundancy_mvp_1-crop.pdf}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}

        \includegraphics[width=\textwidth]{figures/redundancy_best_case_1-crop.pdf}
    \end{subfigure}
    
    \medskip
    \begin{subfigure}{0.015\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_title_vert2-crop.pdf}
        
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_random_2-crop.pdf}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_mvp_2-crop.pdf}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_best_case_2-crop.pdf}
    \end{subfigure}
    
    \medskip
    \begin{subfigure}{0.015\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_title_vert3-crop.pdf}
        
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
    \includegraphics[width=\textwidth]{figures/redundancy_random_3-crop.pdf}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
    \includegraphics[width=\textwidth]{figures/redundancy_mvp_3-crop.pdf}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_best_case_3-crop.pdf}
        \end{subfigure}
    
    \medskip

        
    \hspace{0.4cm}
    \begin{subfigure}{0.12\textwidth}
        \hspace{-0.3cm}
        \includegraphics[width=\textwidth]{figures/redundancy_title_hor1-crop.pdf}
    \end{subfigure}\hspace*{0.7cm}
    \begin{subfigure}{0.09\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/redundancy_title_hor2-crop.pdf}
    \end{subfigure}\hspace*{0.9cm}
    \begin{subfigure}{0.1\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/redundancy_title_hor3-crop.pdf}
        \end{subfigure}

    \caption{Redundancy among a subset of 100 existing VPs selected using three different techniques for three increasingly stricter redundancy definitions. Naively selecting VPs (random, left column) implies collecting data with a high level of redundancy. Selecting VPs with \name enables reducing significantly the level of redundancy among BGP data.}
    \label{fig:redundancy}
\end{figure}


\vspace{-0.15cm}
\subsubsection{\name aims to avoid redundancy}\hfill%
\label{sec:opportunity2}


\fref{fig:redundancy} (left) shows that the VPs can be highly redundant
when they are selected randomly.  For instance, with the loose Def.
\ref{def:red1}, we observe that 83 of the VPs have >50\% of their updates
that are redundant with the ones observed by five other VPs or more
(21 for Def. \ref{def:red2} and 13 for Def. \ref{def:red3}).
\kc{this just means all fullfeed VPs see most of the Internet, right?}
\myitem{\name returns a set 
of VPs that exhibits lower redundancy. }
\fref{fig:redundancy} (middle) shows the level of redundancy
between 100 VPs
returned by \name. Clearly, the level of redundancy is below the one observed 
from 100 randomly selected VPs. With the loose Def. \ref{def:red1}, only 45
of the VPs have >50\% of their updates that are redundant with the ones observed by five other VPs or more.
This number goes down to 11 with Def. \ref{def:red2} and 10 with Def. \ref{def:red3}.



\myitem{The compound of BGP updates collected using \name exhibits low redundancy.}
We examined the compound of BGP updates collected by the 100 VPs selected either randomly or with \name.
We find that 72.5\% of the updates collected by the 100 VPs selected randomly are redundant with at least 
another collected update with Def. \ref{def:red1}. This number goes down to 34\% with Def. \ref{def:red2} and 14.2\%
with Def. \ref{def:red3}. 
Logically, a lower proportion of updates is redundant when collected by a set of VPs selected using \name.
We find that 64.3\% of them are redundant with at least another collected update with Def. \ref{def:red1}.
This number goes down to 23.4\% witg Def. \ref{def:red2} and 12.8\%
with Def. \ref{def:red3}. 














\subsection{Main challenge: prevent overfitting}
\label{sec:challenges}


Our design objective is a general framework that can accommodate
a researcher's given definition of redundancy in selecting
the set of least redundant VPs.  However, optimizing selection
for one objective (i.e., definition) is likely to overfit, leading to
poor performance for other objectives. 
\kc{but within limits right?
must be one of your 3 definitions?  or do you claim more?}
Thus, while the three definitions in \S\ref{sec:opportunity1} enable illustrating the redundancy
among the BGP data, none of them are used in the design of \name. These definitions
are too naive to accurately quantify the redundancies between the VPs.

























We explore this risk of overfitting to a particular objective,
by developing 
three \textit{greedy specific} selection strategies, one for every 
redundancy definition we used in \S\ref{sec:opportunity1}. 
Here, a \textit{greedy specific} approximates an optimal selection
using a greedy approach and returns a set of 100 VPs
that exhibits the lowest level of redundancy (across all the pairs of selected VPs)
for a given redundancy definition. We explain more in detail how we implemented \textit{greedy specific} in \S\ref{sec:eval}. 

\myitem{Logically, greedy specific outperforms \name.}
\textit{greedy specific} slightly outperforms \name and returns
less redundant VPs (see \fref{fig:redundancy}, right).
With the loose Def. \ref{def:red1}, only 6
VPs have >50\% of their updates that are redundant with the ones observed by five other VPs or more.
This number goes down to 0 with Def. \ref{def:red2} and Def. \ref{def:red3}.

\myitem{Unfortunately, greedy specific overfits.}
\textit{Greedy specific} overfits because it is optimized for one particular objective.
Thus, it works well (\ie better than \name) for this objective but not (\ie worse than \name) for the others. 
We confirm this overfitting effect in \S\ref{sec:eval} where we benchmark \textit{greedy specific} against 
\name on various objectives and show that it performs poorly on objectives that it does not optimized.  
Consequently, one would need to design a \textit{greedy specific} VPs selection for every
possible definition of data redundancy---which is unpractical given that there is an infinite number of definitions.








    











==> case_mvp_old.tex <==
\section{The case for \name}
\label{sec:mvp}

We demonstrate the value of strategic selection of VPs from
\ris and \rv (\S\ref{sec:problems}) and show the opportunity 
offered by redundancy in the data (\S\ref{sec:opportunity}) 
that \name leverages (\S\ref{sec:challenges}).


\subsection{Problem}
\label{sec:problems}


Deploying more VPs expands visibility of the routing system
(\S\ref{sec:case1}), but also dramatically increases collected data
volumes, raising barriers to its use (\S\ref{sec:problem2}) which negatively impacts the quality of the data collected by users  
given their unoptimized pratices (\S\ref{sec:problem3}).


\vspace{-0.15cm}
\subsubsection{Deploying more VPs improves data completeness.}\hfill%
\label{sec:case1}




A tiny fraction (1.3\%) of the 74k ASes participating in the global
routing system~\cite{cidr_report} host a VP.
This fraction remains low (X\%) even when focusing on the Y transit (and more connected) ASes.  
Although we cannot
know how much additional topology we might observe from VPs that do not
peer with the public collection systems, \kc{@@get estimate from akamai,
or others?}, we can estimate this gap using simulations of topologies
whose statistical parameters match those of the known global Internet.


\myitem{Methodology.}
We created a mini-Internet with 600 ASes, each running a single BGP
router.  We generated the AS topology using the Hyperbolic Graph
Generator~\cite{ALDECOA2015492}. We set the average node degree to 6.1,
which results in a comparable degree of connectivity (\textit{a.k.a.}
Beta index) to the one observed in CAIDA's AS relationship dataset
from December 2022~\cite{CAIDA_relationships}, and use as the 
degree distribution
a power law with exponent 2.1 (as in~\cite{ALDECOA2015492}).  We defined
the AS relationships as follows. The three ASes with the highest degree
are Tier1 ASes and are fully meshed. ASes directly connected to a Tier1
are Tier2s.  ASes directly connected to a Tier2 but not to a Tier1 are
Tier3s, etc. Two connected ASes have a peer-to-peer (p2p) relationship
if they are on the same level, a customer-to-provider (c2p) relationship
if not.  The routing policies follow the Gao-Rexford model~\cite{GaoRexford}.




\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/mini_internet-crop.pdf}
    \caption{Simulations with a 600-ASes mini-Internet from which we make two key observations:
    \first deploying more VPs helps observing more AS links (especially p2p links), and \second
    arbitrarily selecting VPs performs poorly compared to selecting them with \textit{greedy specific} (a best-base approximation). }
    \label{fig:mini-internet_exp}
\end{figure}%

\fref{fig:mini-internet_exp} shows the proportion of observed AS links
as a function of the number of ASes hosting a VP. We consider 
three VP deployment strategies: \first \textit{random}, which randomly deploys VPs across all the ASes;
\second \textit{distance-based}, which aims to maximize the AS-level distance between the deployed VPs; and \third
\textit{greedy specific}, which approximates the best case using a greedy approach.
We ran every selection strategy twenty times (with different random seeds) and show the results in the boxes.
The line in a box depicts the
median value; the whiskers show the 5 and the 95th percentile.
We computed the proportion of observed links and show separately the 
p2p and 
c2p links in \fref{fig:mini-internet_exp}. 

\myitem{Conclusions.}
Although we take the results with a grain of salt
because the topology differs (but exhibits similar patterns) from the actual (unknown)
AS topology, we tentatively draw the following five conclusions.

\noindent
\Firstp For a given VP deployment strategy, more VPs often leads to more
links observed and all links are observed only when all ASes host a VP.
This result is intuitive as combining local views helps to gather more routing information (see \S\ref{sec:background}).

\noindent
\Secondp P2p links are harder to observe than c2p links.
After investigation, we observe that they are more visible from VPs at the edge,
which aligns with the scenarios depicted in \fref{fig:partial_view}.
Again, this result is intuitive as, unlike c2p links, p2p links are 
not expected to be advertised upwards in the Internet hierarchy when routing policies follow the Gao-Rexford model.

\noindent
\Fourthp The \textit{distance-based} deployment strategy performs poorly (even worse than random deployment).

\noindent
\Fifthp When 1.3\% of ASes host a VP (\ie the same proportion 
as current \ris and \rv VPs), %
only 35\% of the links are observed.

\myitem{Key takeaway.}
Our conclusions suggest that
deploying more VPs improves visible coverage of the routing topology.
Consequently, new deployments of VPs by \ris and \rv can be beneficial,
and we can expect---and hope for---their number to keep increasing (see \fref{fig:ris_nb_vp2}).





\vspace{-0.15cm}
\subsubsection{Deploying more VPs complicates data usability.}\hfill%
\label{sec:problem2}


Deploying more VPs generates more data as each of them collects BGP updates.
Moreover, new IP prefixes advertised in BGP (see~\cite{cidr_report})
increase the volume of data collected by every VP.
In fact, every new IP prefix advertised in BGP triggers the propagation of
new BGP routes that many VPs (\eg the full feeders) observe
and send to the collection platforms.
The compound effect---more VPs (\fref{fig:ris_nb_vp2})
and more updates per VP (\fref{fig:update_vp2})---yields 
a \textit{quadratic} increase in updates reaching the 
collection platforms (\fref{fig:ris_nb_updates}),
which concerns users and data providers~\cite{aben_concern}.
Although several tools aims to speed up the data processing~\cite{bgpstream,bgpkit,9464008},
our literature review revealed that many studies used only a
sample of data collected by \ris and \rv, either using only a subset of the VPs
or a short duration of time, or both.
While authors do not typically explain why they do not use all the data,
the sampling suggests two (inter-related) explanations: authors believe the
sample is representative and sufficiently complete; and/or the data volume is
not worth trying to manage.
We confirm that this is the common behaviors with a survey
that we conducted on authors of ten research papers.  















\myitem{Methodology.} We classified ten BGP-based studies from top
conferences\footnote{SIGCOMM, NSDI, S\&P, USENIX Security, NDSS and IMC. }
into two categories based on how they used BGP data.\footnote{A
	paper may be in both categories.}
Seven papers used \textbf{all} routes collected from 
a \textbf{subset} of the VPs (category $C_1$);  
five papers used a \textbf{short time frame} ($C_2$).
For each paper, we asked the authors questions regarding
their use of BGP data: whether data volume limited their work, 
how and why they sampled BGP data sources, their understanding of
the impact on the quality of their results, and if they would do 
things differently if they had more resources or time.  
We summarize results here; details of the survey are in
an appendix (\S\ref{sec:survey}).

\myitem{The volume of BGP data to process is often a limiting factor.}
Seven (of 9) respondents found the BGP data expensive to process.
For three respondents in $C_1$, processing time motivated them
to use only a subset of the VPs; three respondents in $C_2$ 
considered the processing time when choosing a measurement interval.
Even a respondent that used a Spark cluster found it 
inhibitively time-consuming to process the BGP data. 

\myitem{Respondents in $C_1$ selected VPs somewhat arbitrarily.}
One respondent picked geographically-distant BGP collectors.
Our experiments
(\fref{fig:mini-internet_exp}) and our evaluation (\S\ref{sec:eval})
show that this intuitive strategy often fails to optimize for a given
metric, such as coverage.  Other respondents said they chose VPs randomly,
or those with the highest number of prefixes.  Another responded
unintentionally discarded some VPs, leaving an arbitrarily selected set
in the study.  Two respondents did not remember how they selected VPs.


\vspace{-0.15cm}
\subsubsection{Current practices negatively impact results.}
\label{sec:problem3}


We show using our controlled simulations and our survey that current
practices to reduce the volume of data to process negatively impact the
quality of the results.

\myitem{Selecting VPs arbitrarily performs poorly.}
Our mini-Internet simulation (\S\ref{sec:case1})
shows that arbitrary VPs selection strategies
perform significantly worse than \textit{greedy specific} (a best-case 
approximation) when the goal is to map the AS topology.
For instance, randomly selecting 20 VPs reveals 12\% of the p2p links compared 
to 56\% when selecting them using \textit{greedy specific}---a 4.7$\times$ improvement factor that we highlight in \fref{fig:mini-internet_exp}.
Our evaluation reveals that this performance gap between using an arbitrary VPs selection
strategy and a best-case approach also exists for various other metrics,
\eg hijacks or transient paths detection (\S\ref{sec:eval}).


\myitem{Six respondents in $C_1$ acknowledged that using more VPs would 
improve the quality of their analysis.}
The last respondent was not sure, given the potential redundancy in
the data sources (which he did not analyze). 
Two of the six believed it would not {\em significantly} change 
the conclusion of their measurement studies
(\eg one said that it could help to pinpoint corner cases).
However, six of the 7 authors in $C_1$ affirmed that they would have
used more VPs if they had more resources and time.


\myitem{All respondents in $C_2$ said that extending the duration of
their study would improve the quality of their results.}
One respondent thougt the gain would not be significant;
another said it could help detect rare routing events. 
All respondents in $C_2$ would have extended the duration 
of their observation window given more time and resources. 
\kc{again, this sounds weak.. discuss}













\subsection{Opportunity to Optimize Sampling}
\label{sec:opportunity}

We now propose a systematic framework to characterize
{\em redundancy} across BGP routes collected by the VPs.  
We use the term {\em redundant} to refer to updates with 
similar (or identical, depending on the \textit{redundancy} definition)
attribute values (\S\ref{sec:opportunity1}).
Thus, two redundant VPs, \ie that observe
redundant routes, likely provide similar views over
routing events such as outages, attacks, etc.  \name exploits this
opportunity to identify a set of nonredundant VPs which collects a compound of BGP updates
with a low level of redundancy (\S\ref{sec:opportunity2}).
\kc{i think the precise defn should be something like
"yields the same inference of scope and duration 
of an inferred harm"..}



\vspace{-0.15cm}
\subsubsection{The VPs of \ris and \rv collect redundant routes}
\label{sec:opportunity1}

\setlist{leftmargin=3mm}


We characterize redundancy between pairs of VPs using three different, gradually stricter, 
definitions of redundancy.
We denote $v_i$ the VP $i$ that observes
a set of BGP updates $U_i$. Consider a BGP update $u_{t,p} \in U_i$
with $t$ the time at which the route was observed and $p$ its prefix.
\begin{defn}[prefix based]
    The update $u_{t_1,p_1} \in U_1$ is redundant with the update $u_{t_2,p_2} \in U_2$ if:
    \begin{itemize}
        \setlength\itemsep{-0.1cm}
        \item $\lvert t_1 - t_2 \lvert < 5$ minutes, and $p_1 = p_2$.
   \end{itemize}
    \label{def:red1}
  \end{defn}
\noindent
We choose 5 minutes because it is an approximation of the BGP convergence time~\cite{transientConv}.
We now denote $A_i(t,p)$ the set of AS links in the AS path of the most recent BGP route observed by 
VP $i$ for prefix $p$ at time $t$.
This definition of redundancy might be appropriate when one is merely trying to map as many routed prefixes as possible during a given time window to some AS originating them into the Internet, i.e., path diversity is not of interest. 
\begin{defn}[prefix and as-path based]
    The update $u_{t_1,p_1} \in U_1$ is redundant with the update $u_{t_2,p_2} \in U_2$ if:
    \begin{itemize}
        \setlength\itemsep{-0.1cm}
        \item $\lvert t_1 - t_2 \lvert < 5$ minutes, and $p_1 = p_2$, and
        \item $A_1(t_1, p_1) \setminus A_1(t_1-\epsilon, p_1) \subset A_2(t_2, p_2) \setminus A_2(t_2-\epsilon, p_2)$.
   \end{itemize}
   \label{def:red2}
\end{defn}
\noindent
More casually, the second condition checks whether the changes (operator $\setminus$)
in the AS paths observed by VP $1$ for a given prefix coincide (operator $\subset$) 
with the changes observed by VP $2$ for the same prefix. 

The last definition 
follows the same approach, but adding BGP communities.
We denote $C_i(t,p)$ the set of community values of the most recent BGP route observed by 
VP $i$ for prefix $p$ and at time $t$.
\noindent
\begin{defn}[prefix, as-path, and community-based]
    The update $u_{t_1,p_1} \in U_1$ is redundant with update $u_{t_2,p_2} \in U_2$ if:
    \begin{itemize}
        \setlength\itemsep{-0.1cm}
        \item $\lvert t_1 - t_2 \lvert < 5$ minutes, and $p_1 = p_2$, and
        \item $A_1(t_1, p_1) \setminus A_1(t_1-\epsilon, p_1) \subset A_2(t_2, p_2) \setminus A_2(t_2-\epsilon, p_2)$, and
        \item $C_1(t_1, p_1) \setminus C_1(t_1-\epsilon, p_1) \subset C_2(t_2, p_2) \setminus C_2(t_2-\epsilon, p_2)$.
   \end{itemize}
   \label{def:red3}
\end{defn}
We note that these definitions are asymmetric. 

\myitem{Redundant pairs of VPs exist.}
\fref{fig:redundancy} shows the level of redundancy for the three definitions and
between 100 VPs selected using three different strategies
and computed over the updates observed during two hours on August 1, 2022.
One cell in the matrix indicates the redundancy of the VP on the ordinate with the VP on the abscissa.
We define the redundancy between VP $v_1$ and VP $v_2$ as the proportion of updates observed 
by $v_1$ that are redundant with at least one update observed by $v_2$.
For better visibility, we show the most redundant VPs at the top of the figures.

\fref{fig:redundancy} illustrates that redundant pairs of VPs exist regardless 
of the redundancy definition used. Logically, the stricter the definition, the fewer redundant pairs of VPs.






\begin{figure}[t!] %


    \begin{subfigure}{0.05\textwidth}
        \includegraphics[width=\textwidth]{figures/white.png}
        
    \end{subfigure}
    \begin{subfigure}{0.38\textwidth}
        \hspace{-10cm}

        \includegraphics[width=\textwidth]{figures/redundancy_colorbar-crop.pdf}
    \end{subfigure}
    \hspace{0.5cm}
        
    \medskip

    \begin{subfigure}{0.015\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_title_vert1-crop.pdf}
        
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
    \includegraphics[width=\textwidth]{figures/redundancy_random_1-crop.pdf}
    
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}

        \includegraphics[width=\textwidth]{figures/redundancy_mvp_1-crop.pdf}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}

        \includegraphics[width=\textwidth]{figures/redundancy_best_case_1-crop.pdf}
    \end{subfigure}
    
    \medskip
    \begin{subfigure}{0.015\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_title_vert2-crop.pdf}
        
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_random_2-crop.pdf}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_mvp_2-crop.pdf}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_best_case_2-crop.pdf}
    \end{subfigure}
    
    \medskip
    \begin{subfigure}{0.015\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_title_vert3-crop.pdf}
        
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
    \includegraphics[width=\textwidth]{figures/redundancy_random_3-crop.pdf}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
    \includegraphics[width=\textwidth]{figures/redundancy_mvp_3-crop.pdf}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.145\textwidth}
        \includegraphics[width=\textwidth]{figures/redundancy_best_case_3-crop.pdf}
        \end{subfigure}
    
    \medskip

        
    \hspace{0.4cm}
    \begin{subfigure}{0.12\textwidth}
        \hspace{-0.3cm}
        \includegraphics[width=\textwidth]{figures/redundancy_title_hor1-crop.pdf}
    \end{subfigure}\hspace*{0.7cm}
    \begin{subfigure}{0.09\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/redundancy_title_hor2-crop.pdf}
    \end{subfigure}\hspace*{0.9cm}
    \begin{subfigure}{0.1\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figures/redundancy_title_hor3-crop.pdf}
        \end{subfigure}

    \caption{Redundancy among a subset of 100 existing VPs selected using three different techniques for three increasingly stricter redundancy definitions. Naively selecting VPs (random, left column) implies collecting data with a high level of redundancy. Selecting VPs with \name enables reducing significantly the level of redundancy among BGP data.}
    \label{fig:redundancy}
\end{figure}


\vspace{-0.15cm}
\subsubsection{\name aims to avoid redundancy}\hfill%
\label{sec:opportunity2}


\fref{fig:redundancy} (left) shows that the VPs can be highly redundant
when they are selected randomly.  For instance, with the loose Def.
\ref{def:red1}, we observe that 83 of the VPs have >50\% of their updates
that are redundant with the ones observed by five other VPs or more
(21 for Def. \ref{def:red2} and 13 for Def. \ref{def:red3}).
\kc{this just means all fullfeed VPs see most of the Internet, right?}
\myitem{\name returns a set 
of VPs that exhibits lower redundancy. }
\fref{fig:redundancy} (middle) shows the level of redundancy
between 100 VPs
returned by \name. Clearly, the level of redundancy is below the one observed 
from 100 randomly selected VPs. With the loose Def. \ref{def:red1}, only 45
of the VPs have >50\% of their updates that are redundant with the ones observed by five other VPs or more.
This number goes down to 11 with Def. \ref{def:red2} and 10 with Def. \ref{def:red3}.



\myitem{The compound of BGP updates collected using \name exhibits low redundancy.}
We examined the compound of BGP updates collected by the 100 VPs selected either randomly or with \name.
We find that 72.5\% of the updates collected by the 100 VPs selected randomly are redundant with at least 
another collected update with Def. \ref{def:red1}. This number goes down to 34\% with Def. \ref{def:red2} and 14.2\%
with Def. \ref{def:red3}. 
Logically, a lower proportion of updates is redundant when collected by a set of VPs selected using \name.
We find that 62.3\% of them are redundant with at least another collected update with Def. \ref{def:red1}.
This number goes down to 22.4\% witg Def. \ref{def:red2} and 12.1\%
with Def. \ref{def:red3}. 














\subsection{Main challenge: prevent overfitting}
\label{sec:challenges}


Our design objective is a general framework that can accommodate
a researcher's given definition of redundancy in selecting
the set of least redundant VPs.  However, optimizing selection
for one objective (i.e., definition) is likely to overfit, leading to
poor performance for other objectives. 
\kc{but within limits right?
must be one of your 3 definitions?  or do you claim more?}
Thus, while the three definitions in \S\ref{sec:opportunity1} enable illustrating the redundancy
among the BGP data, none of them are used in the design of \name. These definitions
are too naive to accurately quantify the redundancies between the VPs.

























We explore this risk of overfitting to a particular objective,
by developing 
three \textit{greedy specific} selection strategies, one for every 
redundancy definition we used in \S\ref{sec:opportunity1}. 
Here, a \textit{greedy specific} approximates an optimal selection
using a greedy approach and returns a set of 100 VPs
that exhibits the lowest level of redundancy (across all the pairs of selected VPs)
for a given redundancy definition. We explain more in detail how we implemented \textit{greedy specific} in \S\ref{sec:eval}. 

\myitem{Logically, greedy specific outperforms \name.}
\textit{greedy specific} slightly outperforms \name and returns
less redundant VPs (see \fref{fig:redundancy}, right).
With the loose Def. \ref{def:red1}, only 6
VPs have >50\% of their updates that are redundant with the ones observed by five other VPs or more.
This number goes down to 0 with Def. \ref{def:red2} and Def. \ref{def:red3}.

\myitem{Unfortunately, greedy specific overfits, making it unpracticable.}
\textit{greedy specific} overfits because it is optimized for one particular objective.
Thus, it works well for this objective but not for the others. 
We confirm this overfitting effect in \S\ref{sec:eval} where we show that \textit{greedy specific} performs 
poorly for four other objectives that we found in the literature and that it does not optimized.  
Consequently, one would need to design a \textit{greedy specific} VPs selection for every
possible definition of data redundancy---which is unpractical given that there is an infinite number of possible redundancy definitions.








    











==> evaluation_app.tex <==
\section{Follow-up Evaluation}
\label{sec:eval_follow_up}


\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{.45\textwidth}
        \includegraphics[width=\textwidth]{figures/legend_eval.pdf}
        \vspace*{-3mm}
    \end{subfigure}
    \vfill
    \begin{subfigure}[t]{.47\textwidth}
        \includegraphics[width=\textwidth]{figures/edges_seceval.pdf}
        \vspace*{-3mm}
        \caption{AS level topology mapping.}
        \label{fig:appuc1}
    \end{subfigure}
    \vfill
    \begin{subfigure}[t]{.47\textwidth}
        \includegraphics[width=\textwidth]{figures/transients_seceval.pdf}
        \vspace*{-3mm}
        \caption{Transient paths detection.}
        \label{fig:appuc2}
    \end{subfigure}
    \vfill
    \begin{subfigure}[t]{.47\textwidth}
        \includegraphics[width=\textwidth]{figures/events_seceval.pdf}
        \vspace*{-3mm}
        \caption{BGP events detection.}
        \label{fig:appuc3}
    \end{subfigure}
    \caption{Utility (left) and Volume (right) regarding the number of selected collectors.}
    \label{fig:appucs}
\end{figure}

In this section we will give an additionnal evaluation of \name and the three baselines.
We will present separatly the \textit{utility} and the \textit{volume}, regarding the 
number of selected VP. We will present these two aspects for each of the use cases 
presented in \S \ref{sec:eval}. 

\myitem{AS level topology mapping.} If we look at \fref{fig:appuc1} (left), we can see 
that greedy method performs better than the other VP selection methods. This is not 
surpising, since it corresponds, for this particular use case, to the best case. 
However, if we now take a look at the right of this figure, we can see that greedy is
outperformed by all the other methods. Once again, this is not surprising. Indeed, most
of the time, the VP that discover a high number of AS links are VP that collect a lot of
data.

Still of \fref{fig:appuc1}, we can see that \name performs better than the two other 
techniques when considering the number of discovered links, but also in terms of volume
of collected data. We can also consider that, in some cases, random performs as good as
\name, but this is due to the high variance of this VP selection method. If one is lucky,
it could expect to have good performances, but could also be unlucky and perform poorly,
compared to other VP selection methods.

\myitem{Transient path detection.} When looking at \fref{fig:appuc2}, we can do the same 
conclusion as before: greedy performs better in terms of utility, but is outperformed when
considering the volume. Even if greedy seems to perform well, in term of tradeoff between
utility and volume, random method performs better than greedy. \name returns a good utility,
compared to other techniques. This is mainly due to the low redundancies between the selected
VP. Indeed, having a low redundancy between our collectors allows us to capture different
portion of the Internet, while keeping the volume of collected data under control. Once
again, one can think that random could perform as well as \name, but this is due to the high
variance of random selection.




==> features.tex <==

\section{Topological features}
\label{sec:features}




\tref{tab:descfeatures} lists the topological features that \name uses to
quantify the observation of the Vantage Points (VPs).
As explained in \S\ref{sec:design_quantification},
\name uses both \textit{node-based} features and \textit{pair-based} features.
\textit{Node-based} features relate 
to a node in the graph (\eg average neighbor degree) whereas \textit{pair-based} features
relate to a pair of nodes  (\eg preferential attachment).

We divide \textit{node-based} features into three subcategories: \textit{Centrality metrics}, 
\textit{neighborhood richness}, and \textit{topological pattern}. For a given node $n$,
the first subcategory includes features that evaluate how important and connected $n$ is in the graph.
The second subcategory captures 
information about the properties of the nodes in the neighborhood of $n$. 
The features in the last subcategory identify the topological patterns that include $n$.
We divide \textit{pair-based} features into two subcategories: \textit{Closeness metrics} and
\textit{distance}. The features in the first subcategory compare the two nodes based on their
importance in the graph, whereas the feature in the second subcategory computes the distance between the two nodes.
Five features take into account the weight on the edges. Recall that the weight on a link
corresponds to the number of AS paths that include this link.

We purposively omit some other topological features because they are either
redundant with the used features or because they induce a significant
computational overhead while providing little improvement.
For instance, we do not use the
\textit{betweenness centrality} because it is heavily correlated with the \textit{centrality metrics} that we use already.
The \textit{pageRank} is not used because it is too long to compute on the AS topology 
and does not significantly improve the performance of \name.
We show in \S\ref{sec:feature_usefulness} that all the feature categories that we use are useful
and help to improve the performance of \name for all the use cases.






==> implementation.tex <==
\section{implementation}
\label{sec:implementation}

We implemented \name's internal algorithms in 1600 lines of Python code.
We use the scikit-learn package to compute the clustering and the networkx package
to build the graphs. 
We run \name on a server with 24 CPUs and 64GB of RAM. 
The most time consuming operation when running \name is the computation
of the topological features. It took about five days to compute the 
changes induced on the feature values for the 500 BGP events.
Of course, we emphasize again that users do not need to compute the
feature values themselves but can simply request the selected VPs
using a \texttt{curl} request.

Observe that computing all the feature values is required to bootstrap \name. 
At runtime, \name can compute new feature values as soon as new BGP events are detected,
update the clusters of VPs accordingly and make available to users 
the new list of selected VPs. Additionally, \name can also stop considering
old events. 





==> motivation.tex <==
\section{Problems}


\myitem{There is an exponential increase of redundant data.}
In addition to the increasing number of VPs, we also see more
and more ASes and IP prefixes announced in the Internet~\cite{cidr_report}.
For every new prefix, the VPs observe additional BGP routes. Putting everything
together, the volume of collected data thus exponentially increases over time
(\fref{fig:load}, right). 

While collecting more data is often beneficial, 
it is a problem with the BGP data because there are more and more
redundant routes due to the highly skewed location of the VPs.
Indeed, VPs are likely positioned in the core of the Internet,
whereas the edge is less covered. For instance, 62\% of the
RIPE RIS VPs are located in the top 5k ASes.

We thus argue that the processing overhead induced by this exponential 
increase prevents users from processing the entire dataset of BGP routes, 
even when focusing on a limited period of time.
As an illustration, Luckie \etal only download a snapshot of the BGP routes
from every VPs \emph{one time} per day for the \emph{first five days} of every month
to maintain the very popular CAIDA's AS relationship dataset~\cite{Luckie2013}.

\myitem{The less data is collected, the more information is missing.}
Because processing all the data is often too expensive in time and resources,
users often download data from a limited number
of VPs. However, collecting routes from a subset of the VPs
inevitably results in less accurate information. Indeed, because BGP is a policy-based
path-vector protocol, it inherently hides part of the existing routes to the VPs. 
Consequently, VPs exhibit highly different partial views over the routes.
Selecting a few of them results in missing many routes and updates only observed 
from the non-selected VPs.



Consider the scenario depicted in \fref{fig:aslevel_topo}
and assume the ASes configure routing policies
following their business relationships~\cite{GaoRexford}.
In this case, VP1 does not see the links
\mbox{\circledl{2} \link \circledl{3}},
\mbox{\circledl{6} \link \circledl{7}} and
\mbox{\circledl{6} \link \circledl{8}}.
Similarly, VP2 does not see the links
\mbox{\circledl{1} \link \circledl{3}},
\mbox{\circledl{2} \link \circledl{7}} and
\mbox{\circledl{3} \link \circledl{8}}.
Thus, it is unsurprising that a study reveals that
53\% of the BGP hijacks and misoriginations were detected by fewer
than 30 VPs in 2020~\cite{manrs_security}.

\myitem{The selection of a right set of VPs is hard.}
Unfortunately, still far too often, users randomly select their VPs.
Clearly, given the highly skewed position of the VPs,
a random selection returns many VPs located within the core
of the Internet, resulting in many edge routes and updates being off the radar.
The problem is that finding a better VP selection strategy is hard: even a 
not so naive approach based on maximizing
the AS-level distance between the selected VPs performs poorly.



We confirmed that the AS-level distance is not a good indicator
to assess the similarity between two VPs with a study
that compares, for 1000 pairs of VPs distant by $n$ AS hops with $n=\{0,1,2,3\}$,
the number of links that they find. 
We found that 15\% of the pairs within the same AS ($n=0$) see more links 
than 31\% of the pairs distant by one hop, 26\% of the pairs distant by two hops
and 15\% of the pairs distant by three hops.
Thus, not so rarely,
VPs located in the same AS see very different AS links,
and vice versa, distant VPs may see a very similar set of AS links. 
While this may seem counterintuitive, we argue that it is the result of the
confidential routing policies and the inaccurate view of
the AS topology measured from the VPs provided by RIPE RIS and that we use
to compute the distance between the VPs.



==> overview.tex <==

\section{Overview}
\label{sec:solution}


In this section, we give an overview of the \name workflow
(\S\ref{sec:solution_overview}), its key ingredients
(\S\ref{sec:solution_practice}), and functions (\S\ref{sec:functions}).
\kc{would turn this into short section providing 
intuition. 




\subsection{Workflow}
\label{sec:solution_overview}

As a path-vector protocol, BGP \textit{hides} information
(\eg backup routes), including sometimes \textit{confidential}
routing policies. 
Thus, \name relies on an inferential process comprising
four phases:  

\myitem{Select a large, unbiased set of BGP events (\S\ref{sec:design_events}).}
\name evaluates the redundancy between two VPs based on topological changes.
To do this, \name relies on past, local, and easily-identifiable events that it chooses carefully.
More precisely, these events are AS-path changes
visible by a few VPs (but not all) 
to allow discriminating what they observe.
\name uses a \textit{large} set of events scattered across \textit{time}
(enabling stability over time, see \S\ref{sec:eval_stability}) and \textit{location}
(preventing overfitting due to routing biases (\S\ref{sec:solution_practice})
to evaluate what every VP sees.


\myitem{Quantification of the observation of the VPs (\S\ref{sec:design_quantification}).}
\kc{propose delete below, replace w one sentence:
Gauging the observation of every VP enables
comparing them---a necessary operation to calculate their redundancy.
As there is no simple formula that quantifies the observation of the VPs,
\name uses its own technique that is motivated
by the information carried in a BGP update (see \S\ref{sec:background}).
More precisely, }
For every BGP event, \name quantifies topological features
(\textit{a.k.a.} network statistics~\cite{nature_2019}) of the
ASes involved as observed from each VP (\ie the
\textit{local views}).  \name relies on topological features
as they embed information about the four attributes of a BGP
update: time, prefix, AS path, and communities. 
\kc{why is it "thus" in this sentence? you haven't 
demonstrated that or even argued it? 
Thus, \name
is efficient regardless of which attribute matters in the
study.  We confirm this in \S\ref{sec:eval_performance}.
}
\kc{above paragraph did not explain to me how it 
"quantifies observation of the VPs", need one crisp sentence here
instead of all this text please}





\myitem{Compute redundancy between VPs (\S\ref{sec:design_similarity}).}
Computing a \textit{redundancy score} between \textit{every} pair of VPs
requires computing the pairwise euclidean distance in a $n$-dimensional space, 
with $n$ depending on the number of topological features and chosen events.
\kc{depending on or that {\em is} n?} 
Intuitively, two VPs that observe the same topological features 
for many diverse BGP events are close in the $n$-dimensional space 
and thus likely redundant.  Besides, \name considers 
the average Euclidean distances \kc{between a pair of VPs} 
computed over different 
and nonoverlapping time periods to mitigate time biases.
\kc{seems to me some features matter more than others in
thinking about redundancy,, this section needs to explain
how this computation differs for the 3 defns}



\myitem{Generate a set with the least redundant (most valuable) VPs (\S\ref{sec:design_generation}).}
\name relies on a greedy algorithm that considers both data \textit{redundancy} and 
its \textit{volume} to build a set that contains the most valuable VPs.
\kc{doesn't like "MV" here, need more precision for what we 
mean by valuable, need quantitative metric}
More precisely, it starts with a singleton that includes the least
redundant VP,
\kc{how is that defined for the first one?  most prefixes? most AS paths?} 
and then greedily adds the VP that provides the best balance between 
how redundant it is with the already selected VPs and the estimated
volume of data that it generates.  Intuitively, the less redundant VPs
that provide a high number of BGP updates are added first whereas the
highly redundant VPs that provide a small number of updates are avoided.
\kc{is there a formula for this balance?  point to section where
it's described later?}


\subsection{Key ingredients}
\label{sec:solution_practice}

We now describe three key ingredients in the design of \name.
\kc{should this section not come before 4.1?}

\myitem{Balanced event selection strategy.}
The location of AS-path changes (the events used by \name to evaluate redundancy)
\kc{define "location of AS path changes" and "skewed"?}
often exhibits biases because of 
the hierarchical structure of the AS topology
and the skewed position of the VPs~\cite{RIS_pavlos}.
To make \name robust against these biases, we design an
event selection strategy that classifies routing events in 
different---and carefully chosen---categories 
\kc{carefully chosen by who? how? which categories}
and selects an equal number of events in every category.
We illustrate the gain of our balanced selection 
compared to a random selection in \S\ref{sec:eval_soundness}.
\kc{we cannot put key parts of our argument in an appendix..}


\myitem{Wide range of topological features.}
Topological features can be used to compare the structural
characteristics of two graphs
(\cite{nature_2019}), which is a comparable problem 
to what \name does when evaluating redundancy.
\name a combines a set of features (\tref{tab:descfeatures}) 
that capture diverse properties of ASes involved in routing events. 
\kc{deleted above, we cannot ref to an appendix as part of argument,
move table 4 back here into paper please. probably all of appendix B has
to come back up in the paper, this is where some of science content is?} 





\myitem{Optimizing the tradeoff between volume and utility.}
Data volumes from different VPs vary widely (\fref{fig:update_vp2}), \eg
full feed export more updates than partial feed.
\name considers the average volume of data collected by every VP, 
and thus 
optimizes the \textit{proportion} of redundant updates 
collected by the selected VPs instead of the absolute number.
We evaluate the tradeoff \name makes between utility of collected data 
and its volume for various objectives in \S\ref{sec:eval}.
\kc{what objective? need more precision here} 


\subsection{Software implementation}
\label{sec:functions}

\kc{should this not be up in 4.1?}

\name runs on a commodity server.
Upon launch, it computes the redundancy between every pair 
of VPs at a yearly granularity. Redundancy between two VPs 
remains stable over time (\S\ref{sec:eval_stability}).
\kc{that sentence goes elsewhere, in science/insight/empirics
part rather than in a software section}
Once ready, \name takes as input a \textit{year}
and a \textit{volume of data} and returns a set of  VPs that generates
a volume of data lower than the one specified as input.
\name returns the redundancy scores
calculated for every pair of VPs.
Thus, users have the option to compute their own set
of complementary VPs based on these redundancy scores and some additional constraints that they might have.
This is useful when users want to include (or exclude) some VPs (regardless of how redundant they are), 
which will result in another set of VPs rather than the default set
provided by \name.
For instance, when measuring routing detours within a particular country, 
a user may want to take all the VPs within the country and some
additional VPs selected by \name. 
\name runs as a service at \website allowing users 
to get a list of VPs without computational expenses.
\kc{should it be integrated into bgp2go? how much work?} 








